Robotouille: An Asynchronous Planning Benchmark for LLM Agents

Effective asynchronous planning, or the ability to efficiently reason and plan over states and actions that must happen in parallel or sequentially, is essential for agents that must account for time delays, reason over diverse long-horizon tasks, and collaborate with other agents. While large language model (LLM) agents show promise in high-level task planning, current benchmarks focus primarily on short-horizon tasks and do not evaluate such asynchronous planning capabilities. We introduce Robotouille, a challenging benchmark environment designed to test LLM agents' ability to handle long-horizon asynchronous scenarios. Our synchronous and asynchronous datasets capture increasingly complex planning challenges that go beyond existing benchmarks, requiring agents to manage overlapping tasks and interruptions. Our results show that ReAct (gpt4-o) achieves 47% on synchronous tasks but only 11% on asynchronous tasks, highlighting significant room for improvement. We further analyze failure modes, demonstrating the need for LLM agents to better incorporate long-horizon feedback and self-audit their reasoning during task execution. Code is available at https://github.com/portal-cornell/robotouille.

==> figures/JSONs/additional_jsons.tex <==
\begin{figure}[ht]
    \centering
    % Left column (longest JSON)
    \noindent
    \begin{minipage}[t]{0.48\textwidth}  % Left column (long JSON)
        \vspace{0pt}  % Align at the top of the column
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
{
    "version": "1.0.0",

    "player": {
        "robot": {
            "front": "robot_front.png",
            "back": "robot_back.png",
            "left": "robot_left.png",
            "right": "robot_right.png"
        }
    },

    "floor": "floorkitchen.png",

    "item": {
        "constants": {
            "STATION_ITEM_OFFSET" : 0.25,
            "X_SCALE_FACTOR": 0.125,
            "Y_SCALE_FACTOR": 0.75
        },
        "entities": {
            "chicken": {
                "assets": {
                    "default": "chicken.png",
                    "cooked": {
                        "asset": "cookedchicken.png",
                        "predicates": ["iscooked"]
                    },
                    "fried": {
                        "asset": "friedchicken.png",
                        "predicates": ["isfried"]
                    }
                },
                "constants": {}
            }, ...
        }
    },

    "station": {
        "constants": {},
        "entities": {
            "fryer": {
                "assets": {
                    "default": "fryer.png"
                },
                "constants": {}
            },...
        }
    },
}
        \end{minted}
        \end{tcolorbox}
    \end{minipage}
    \hfill
    % Right column (stacked two JSONs)
    \begin{minipage}[t]{0.48\textwidth}  % Right column
        \vspace{0pt}
        % First stacked JSON
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
{
    "version": "1.0.0",
    "width": 3,
    "height": 3,
    "config": {
        "num_cuts": {
            "lettuce": 3,
            "default": 3
        },
        "cook_time": {
            "patty": 3,
            "default": 3
        }
    },
    "stations": [
        {
            "name": "board",
            "x": 0,
            "y": 1,
            "id": "A"
        }
    ],
    "items": [
        {
            "name": "lettuce",
            "x": 0,
            "y": 1,
            "stack-level": 0,
            "predicates": ["iscuttable"],
            "id": "a"
        }
    ],
    "players": [
        {
            "name": "robot",
            "x": 0,
            "y": 0,
            "direction": [0, 1]
        }
    ],
    "goal_description": "Cut the lettuce on the board until it is cut",
    "goal": [
        {
            "predicate": "iscut",
            "args": ["lettuce"],
            "ids": ["a"]
        }
    ]
}
        \end{minted}
        \end{tcolorbox}

        \vspace{1em}  % Space between stacked JSONs

        % Second stacked JSON
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
{
    "mouse_click_actions": [
        {
            "name": "move",
            "input_instructions": {
                "button": "left",
                "click_on": "s2"
            }
        },...
    ],
    "keyboard_actions": [
        {
            "name": "cook",
            "input_instructions": {
                "key": "e",
                "at": "s1"
            }
        },...
    ]
}
        \end{minted}
        \end{tcolorbox}
    \end{minipage}
    
    \caption{Combined JSONs: (Left) Rendering JSON, (Top-right) Environment JSON, (Bottom-right) Input JSON.}
    \label{fig:combined_jsons}
\end{figure}

==> figures/JSONs/env_json.tex <==
\begin{figure}[t!]
    \centering
    \noindent
    \begin{minipage}[t]{0.8\textwidth}  % Full width minipage
        \vspace{0pt}  % Ensure alignment at the top of the column
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"width": 3,
"height": 3,
"config": {
    "num_cuts": {
        "lettuce": 3,
        "default": 3
    },
    "cook_time": {
        "patty": 3,
        "default": 3
}},
"stations": [{
    "name": "board",
    "x": 0,
    "y": 1,
    "id": "A"
}],
"items": [{
    "name": "lettuce",
    "x": 0,
    "y": 1,
    "stack-level": 0,
    "predicates": ["iscuttable"],
    "id": "a"
}],
"players": [{
    "name": "robot",
    "x": 0,
    "y": 0,
    "direction": [0, 1]
}],
"goal_description": "Cut the lettuce on the board until it is cut",
"goal": [{
    "predicate": "iscut",
    "args": ["lettuce"],
    "ids": ["a"]
}]
        \end{minted}
        \end{tcolorbox}
    \end{minipage}
    \caption{Environment JSON for a lettuce cutting task.}
    \label{fig:environment_json_example}
\end{figure}

==> figures/JSONs/fig_json_compressed.tex <==
\noindent
\begin{minipage}[t]{0.48\textwidth}  % First column for JSON 1 and JSON 3
    \vspace{0pt}  % Ensure alignment at the top of the column
    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"sfx": [{"type": "cond", "param": "i1",
  "conds": [{"pred": "item_on", "params": ["i1", "s1"], "true": true}],
  "fx": [{"pred": "iscooking", "params": ["i1"], "true": true}],
  "sfx": [{"type": "delayed", "param": "i1", "fx": [
    {"pred": "iscooked", "params": ["i1"], "true": true},
    {"pred": "iscooking", "params": ["i1"], "true": false}],
  "sfx": []}]
}]
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(a) Nested special effects for 'cook' action}
    \end{center}
    
    \vspace{-1em} % Adjust vertical spacing between the two boxes

    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"pred_defs": [{"name": "istable", "param_types": ["station"],
  "lang_desc": {"0": "{0} is a table"}},
  {"name": "item_on", "param_types": ["item", "station"],
  "lang_desc": {"0": "{0} on {1}", "1": "{1} has {0} on top"}}]
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(c) Predicate Definitions.}
    \end{center}
\end{minipage}
\hfill  % Horizontal space between the columns
\begin{minipage}[t]{0.48\textwidth}  % Second column for JSON 2 and JSON 4
    \vspace{0pt}  % Ensure alignment at the top of the column
    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"goal_desc": "Prepare a cheeseburger on a table",
"goal": [{"pred": "item_on", "args": ["bottombun", "table"], "ids": [1, 2]},
  {"pred": "item_at", "args": ["cheese", "table"], "ids": [3, 2]},
  {"pred": "item_at", "args": ["patty", "table"], "ids": [4, 2]},
  {"pred": "item_at", "args": ["topbun", "table"], "ids": [5, 2]},
  {"pred": "clear", "args": ["topbun"], "ids": [5]}]
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(b) Goal Description.}
    \end{center}
    
    \vspace{-1em} % Adjust vertical spacing between the two boxes

    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"name": "move", "precons": [{"pred": "loc", "params": ["p1", "s1"], "true": true}],
"imm_fx": [{"pred": "loc", "params": ["p1", "s2"], "true": true},
  {"pred": "loc", "params": ["p1", "s1"], "true": false}],
"sfx": [], "lang_desc": "Move {p1} from {s1} to {s2}"
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(d) Action Definitions.}
    \end{center}
\end{minipage}


==> figures/JSONs/fig_json_final.tex <==
\begin{figure}[!h]
    \centering
    \noindent
    \begin{minipage}[t]{0.48\textwidth}  % First column for JSON 1 and JSON 3
        \vspace{0pt}  % Ensure alignment at the top of the column
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"predicate_defs": [{
  "name": "istable",
  "param_types": ["station"],
  "language_descriptors": {
      "0": "{0} is a table"
  }},{
  "name": "item_on",
  "param_types": ["item", "station"],
  "language_descriptors": {
    "0": "{0} is directly on top of {1}",
    "1": "{1} has {0} directly on top of it"
}},...]
        \end{minted}
        \end{tcolorbox}
        \begin{center}
            \footnotesize \textit{(a) Predicate Definitions}
        \end{center}
        
        \vspace{-1em} % Adjust vertical spacing between the two boxes
    
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"sfx": [{
  "type": "conditional",
  "param": "i1",
  "conditions": [{
    "predicate": "item_on",
    "params": ["i1", "s1"],
    "is_true": true
  }],
  "fx": [{
    "predicate": "iscooking",
    "params": ["i1"],
    "is_true": true
  }],
  "sfx": [{
    "type": "delayed",
    "param": "i1",
    "fx": [{
      "predicate": "iscooked",
      "params": ["i1"],
      "is_true": true
    }, {
      "predicate": "iscooking",
      "params": ["i1"],
      "is_true": false
    }],
    "sfx": []
  }]
}]
        \end{minted}
        \end{tcolorbox}
        \begin{center}
            \footnotesize \textit{(c) Nested special effects for 'cook' action}
        \end{center}
    \end{minipage}
    \hfill  % Horizontal space between the columns
    \begin{minipage}[t]{0.48\textwidth}  % Second column for JSON 2 and JSON 4
        \vspace{0pt}  % Ensure alignment at the top of the column
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"name": "move",
"precons": [{
  "predicate": "loc",
  "params": ["p1", "s1"],
  "is_true": true
}, ...],
"immediate_fx": [{
    "predicate": "loc",
    "params": ["p1", "s2"],
    "is_true": true
  }, {
    "predicate": "loc",
    "params": ["p1", "s1"],
    "is_true": false
  }, ...],
"sfx": [],
"language_description": "Move {p1} from {s1} to {s2}"
        \end{minted}
        \end{tcolorbox}
        \begin{center}
            \footnotesize \textit{(b) Action Definitions}
        \end{center}
        
        \vspace{-1em} % Adjust vertical spacing between the two boxes
    
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"goal_description": "Make lettuce cheese sandwich on table",
"goal": [{
    "predicate": "item_on",
    "args": ["bread", "table"],
    "ids": [1, 2]
  }, {
    "predicate": "item_at",
    "args": ["lettuce", "table"],
    "ids": [3, 2]
  }, {
    "predicate": "item_at",
    "args": ["cheese", "table"],
    "ids": [4, 2]
  }, {
    "predicate": "item_at",
    "args": ["bread", "table"],
    "ids": [5, 2]
  }, {
    "predicate": "clear",
    "args": ["bread"],
    "ids": [5]
}]
        \end{minted}
        \end{tcolorbox}
        \begin{center}
            \footnotesize \textit{(d) Goal Description}
        \end{center}
    \end{minipage}
    \caption{\robotouille{} uses domain and problem JSONs to define the MDP and language description of an environment and tasks using (a) predicate definitions, (b) action definitions, (c) special action effects and (d) goal definitions. See Appendix~\ref{app:additional-jsons} for other JSONs used.}
    \label{fig:jsons}
\end{figure}


==> figures/JSONs/fig_json_no_headers.tex <==
\noindent
\begin{minipage}[t]{0.48\textwidth}  % First column for JSON 1 and JSON 3
    \vspace{0pt}  % Ensure alignment at the top of the column
    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"sfx": [{
  "type": "conditional",
  "param": "i1",
  "conditions": [{
    "predicate": "item_on",
    "params": ["i1", "s1"],
    "is_true": true
  }],
  "fx": [{
    "predicate": "iscooking",
    "params": ["i1"],
    "is_true": true
  }],
  "sfx": [{
    "type": "delayed",
    "param": "i1",
    "fx": [{
      "predicate": "iscooked",
      "params": ["i1"],
      "is_true": true
    }, {
      "predicate": "iscooking",
      "params": ["i1"],
      "is_true": false
    }],
    "sfx": []
  }]
}]
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(a) Nested special effects for 'cook' action}
    \end{center}
    
    \vspace{-1em} % Adjust vertical spacing between the two boxes

    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"predicate_defs": [{
  "name": "istable",
  "param_types": ["station"],
  "language_descriptors": {
      "0": "{0} is a table"
  }},{
  "name": "item_on",
  "param_types": ["item", "station"],
  "language_descriptors": {
    "0": "{0} is directly on top of {1}",
    "1": "{1} has {0} directly on top of it"
}},...]
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(c) Predicate Definitions.}
    \end{center}
\end{minipage}
\hfill  % Horizontal space between the columns
\begin{minipage}[t]{0.48\textwidth}  % Second column for JSON 2 and JSON 4
    \vspace{0pt}  % Ensure alignment at the top of the column
    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"goal_description": "Prepare a cheeseburger on a table",
"goal": [{
    "predicate": "item_on",
    "args": ["bottombun", "table"],
    "ids": [1, 2]
  }, {
    "predicate": "item_at",
    "args": ["cheese", "table"],
    "ids": [3, 2]
  }, {
    "predicate": "item_at",
    "args": ["patty", "table"],
    "ids": [4, 2]
  }, {
    "predicate": "item_at",
    "args": ["topbun", "table"],
    "ids": [5, 2]
  }, {
    "predicate": "clear",
    "args": ["topbun"],
    "ids": [5]
}]
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(b) Goal Description.}
    \end{center}
    
    \vspace{-1em} % Adjust vertical spacing between the two boxes

    \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"name": "move",
"precons": [{
  "predicate": "loc",
  "params": ["p1", "s1"],
  "is_true": true
}, ...],
"immediate_fx": [{
    "predicate": "loc",
    "params": ["p1", "s2"],
    "is_true": true
  }, {
    "predicate": "loc",
    "params": ["p1", "s1"],
    "is_true": false
  }, ...],
"sfx": [],
"language_description": "Move {p1} from {s1} to {s2}"
    \end{minted}
    \end{tcolorbox}
    \begin{center}
        \footnotesize \textit{(d) Action Definitions.}
    \end{center}
\end{minipage}

==> figures/JSONs/fig_json_with_headers.tex <==
% Two columns side by side
\noindent
\begin{minipage}[t]{0.48\textwidth}  % First column for JSON 1 and JSON 3
    \vspace{0pt}  % Ensure alignment at the top of the column
    \begin{tcolorbox}[title=(a) JSON 1: SFX Conditional, colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"sfx": [{
  "type": "conditional",
  "param": "i1",
  "conditions": [{
    "predicate": "item_on",
    "params": ["i1", "s1"],
    "is_true": true
  }],
  "fx": [{
    "predicate": "iscooking",
    "params": ["i1"],
    "is_true": true
  }],
  "sfx": [{
    "type": "delayed",
    "param": "i1",
    "fx": [{
      "predicate": "iscooked",
      "params": ["i1"],
      "is_true": true
    }, {
      "predicate": "iscooking",
      "params": ["i1"],
      "is_true": false
    }],
    "sfx": []
  }]
}]
    \end{minted}
    \end{tcolorbox}
    
    \vspace{-1em} % Adjust vertical spacing between JSON 1 and JSON 3

    \begin{tcolorbox}[title=(c) JSON 3: Predicate Definitions, colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"predicate_defs": [{
  "name": "istable",
  "param_types": ["station"],
  "language_descriptors": {
      "0": "{0} is a table"
  }},{
  "name": "item_on",
  "param_types": ["item", "station"],
  "language_descriptors": {
    "0": "{0} is directly on top of {1}",
    "1": "{1} has {0} directly on top of it"
}},...]
    \end{minted}
    \end{tcolorbox}
\end{minipage}
\hfill  % This will create horizontal space between the two columns
\begin{minipage}[t]{0.48\textwidth}  % Second column for JSON 2 and JSON 4
    \vspace{0pt}  % Ensure alignment at the top of the column
    \begin{tcolorbox}[title=(b) JSON 2: Goal Description, colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"goal_description": "Prepare a cheeseburger on a table",
"goal": [{
    "predicate": "item_on",
    "args": ["bottombun", "table"],
    "ids": [1, 2]
  }, {
    "predicate": "item_at",
    "args": ["cheese", "table"],
    "ids": [3, 2]
  }, {
    "predicate": "item_at",
    "args": ["patty", "table"],
    "ids": [4, 2]
  }, {
    "predicate": "item_at",
    "args": ["topbun", "table"],
    "ids": [5, 2]
  }, {
    "predicate": "clear",
    "args": ["topbun"],
    "ids": [5]
}]
    \end{minted}
    \end{tcolorbox}
    
    \vspace{-1em} % Adjust vertical spacing between JSON 2 and JSON 4

    \begin{tcolorbox}[title=(d) JSON 4: Action Definitions, colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
    \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
        xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
        highlightlines=true, style=colorful, 
        highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"name": "move",
"precons": [{
  "predicate": "loc",
  "params": ["p1", "s1"],
  "is_true": true
}, ...],
"immediate_fx": [{
    "predicate": "loc",
    "params": ["p1", "s2"],
    "is_true": true
  }, {
    "predicate": "loc",
    "params": ["p1", "s1"],
    "is_true": false
  }, ...],
"sfx": [],
"language_description": "Move {p1} from {s1} to {s2}"
    \end{minted}
    \end{tcolorbox}
\end{minipage}

% Add a caption or figure note
\begin{center}
    \footnotesize \textit{Figure 1: Layout example with JSON data in two columns with colored keys and values using minted.}
\end{center}

==> figures/JSONs/input_json.tex <==
\begin{figure}[t!]
    \centering
    \noindent
    \begin{minipage}[t]{0.96\textwidth}  % Full width minipage
        \vspace{0pt}  % Ensure alignment at the top of the column
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}

"mouse_click_actions": [{
    "name": "move",
    "input_instructions": {
        "button": "left",
        "click_on": "s2"
    }},...],
"keyboard_actions": [{
    "name": "cook",
    "input_instructions": {
        "key": "e",
        "at": "s1"
    }},...]

        \end{minted}
        \end{tcolorbox}
    \end{minipage}
    \caption{Input JSON.}
    \label{fig:input_json_example}
\end{figure}

==> figures/JSONs/rendering_json.tex <==
\begin{figure}[t!]
    \centering
    \noindent
    \begin{minipage}[t]{0.96\textwidth}  % Full width minipage
        \vspace{0pt}  % Ensure alignment at the top of the column
        \begin{tcolorbox}[colframe=black, boxrule=0.5mm, width=\textwidth, boxsep=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt]
        \begin{minted}[fontsize=\scriptsize, breaklines, frame=none, bgcolor=white,
            xleftmargin=0pt, xrightmargin=0pt, texcomments=true, escapeinside=||,
            highlightlines=true, style=colorful, 
            highlightcolor=\color{red}, highlightcolor=\color{green}] {json}
"player": {
    "robot": {
        "front": "robot_front.png",
        "back": "robot_back.png",
        "left": "robot_left.png",
        "right": "robot_right.png"
    }},
"floor": "floorkitchen.png",
"item": {
    "constants": {
        "STATION_ITEM_OFFSET" : 0.25,
        "X_SCALE_FACTOR": 0.125,
        "Y_SCALE_FACTOR": 0.75
    },
    "entities": {
        "chicken": {
            "assets": {
                "default": "chicken.png",
                "cooked": {
                    "asset": "cookedchicken.png",
                    "predicates": ["iscooked"]
                },
                "fried": {
                    "asset": "friedchicken.png",
                    "predicates": ["isfried"]
                }
            },
            "constants": {}
        }, ...}},
"station": {
    "constants": {},
    "entities": {
        "fryer": {
            "assets": {
                "default": "fryer.png"
            },
            "constants": {}
        },...}}
        \end{minted}
        \end{tcolorbox}
    \end{minipage}
    \caption{Rendering JSON.}
    \label{fig:rendering_json_example}
\end{figure}

==> figures/first_draft/fig_histogram_optimality.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\textwidth]{assets/first_draft/FINAL_optimality.png}
    \caption{Histogram of the optimality rate for synchronous and asynchronous datasets. The 1 bin includes attempts that were optimal. Attempts between $(1, 1.5]$ are suboptimal but classified as successful. Attempts greater than an optimality rate of 1.5 are classified as failures.
    % \GG{Yuki suggests a proportional histogram would make more sense due to unequal data sizes}
    }
    \label{fig:histogram_optimality}
\end{figure}

==> figures/first_draft/fig_histogram_repeated_actions.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\textwidth]{assets/first_draft/FINAL_repeated_actions.png}
    \caption{\GG{update figure x-axis from actions to transitions} Histogram of the repeated transitions on the synchronous and asynchronous datasets. Green bars represent successes and red bars represent failures.}
    \label{fig:histogram_repeated_transitions}
\end{figure}

==> figures/first_draft/fig_histogram_steps_to_go.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\textwidth]{assets/first_draft/FINAL_steps_to_go.png}
    \caption{Histogram of the normalized steps to go for synchronous and asynchronous datasets. The 0 to 0.5 bucket includes attempts that were making progress towards the goal while the 0.5 to 1 bucket includes attempts that made little to no progress towards the goal. Buckets greater than 1 includes attempts that traversed further away from the goal.
    \YW{You should put numbers above the histogram instead of telling the number in your analysis paragraph.}
    % \GG{Yuki suggests a proportional histogram would make more sense due to unequal data sizes}
    }
    \label{fig:histogram_steps_to_go}
\end{figure}

==> figures/first_draft/fig_piechart_taxonomy.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{assets/first_draft/FINAL_piecharts.png}
    \caption{Nested pie chart of \gptfo{} \react{} failure modes capturing uncertainties in the MDP. The main categories are on the outer circle representing the uncertainty in the state space (S), action space (A), transition function (T), or reward/goal (G). The subcategories on the inner circle represent the dominant cause of failure and are described further in Appendix~\ref{app:taxonomy-details}.}
    \label{fig:piechart_taxonomy}
\end{figure}

==> figures/second_draft/fig_histogram_optimality.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\textwidth]{assets/second_draft/optimality_fixed.png}
    \caption{Histogram of the optimality rate for \gptfo{} \react{} successes on the synchronous and asynchronous datasets. The 1 bin includes attempts that were optimal. Attempts between $(1, 1.5]$ are suboptimal but classified as successful. Attempts greater than an optimality rate of 1.5 are classified as failures.
    % \GG{Yuki suggests a proportional histogram would make more sense due to unequal data sizes}
    % \YW{nitpick: all your plots with numbers could really benefit from increasing the font of the numbers}
    }
    \label{fig:histogram_optimality}
\end{figure}

==> figures/second_draft/fig_histogram_repeated_transitions.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\textwidth]{assets/second_draft/repeated_transitions_better.png}
    \caption{Histogram of the repeated transitions of \gptfo{} \react{} runs on the synchronous and asynchronous datasets. The median separates the data into runs with lower and higher repeated transitions and the quartiles represent the mean of these two groups.}
    \label{fig:histogram_repeated_transitions}
\end{figure}

==> figures/second_draft/fig_histogram_steps_to_go.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\textwidth]{assets/second_draft/steps_to_go.png}
    \caption{Histogram of the normalized steps to go for \gptfo{} \react{} failures on the synchronous and asynchronous datasets. The 0 to 0.5 bucket includes attempts that were making progress towards the goal while the 0.5 to 1 bucket includes attempts that made little to no progress towards the goal. Buckets greater than 1 includes attempts that traversed further away from the goal.
    % \YW{You should put numbers above the histogram instead of telling the number in your analysis paragraph.}
    % \GG{Yuki suggests a proportional histogram would make more sense due to unequal data sizes}
    }
    \label{fig:histogram_steps_to_go}
\end{figure}

==> figures/second_draft/fig_piechart_followup.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{assets/second_draft/follow-up-piechart-prior.png}
    \caption{Nested pie chart of failure modes capturing uncertainties in the MDP of \gptfo{} \reactp{} on Tasks 1 to 3 (30 problems) of the asynchronous dataset using \gptfo{} \react{} and \gptfo{} \reactp{}.}
    \label{fig:piechart_followup}
\end{figure}

==> figures/second_draft/fig_piechart_taxonomy.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{assets/second_draft/bad-start-piechart.png}
    \caption{Nested pie chart of \gptfo{} \react{} failure modes capturing uncertainties in the MDP. The main categories are on the outer circle representing the uncertainty in the state space (S), action space (A), transition function (T), or reward/goal (G). The subcategories on the inner circle represent the dominant cause of failure and are described further in Appendix~\ref{app:taxonomy-details}.}
    \label{fig:piechart_taxonomy}
\end{figure}

==> figures/table_2_task_performance_oldimages.tex <==
% % Table looks weird in terms of multiples of 10

\begin{table}[h]
    \small
    \centering
    \begin{tabular}{llll|l}
        \toprule
        & \textbf{I/O} & \textbf{I/O CoT} & \textbf{ReAct} & \textbf{Horizon} \\
        & & & & \textbf{Length} \\
        \midrule
        \multicolumn{5}{c}{\textbf{Synchronous}} \\
        \midrule
        $\hyperref[fig:0_sync]{[1 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/1_sync.png}  & 20 & 40 & \textbf{70} & 10       \\
        $\hyperref[fig:1_sync]{[2 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/2_sync.png}  & 0  & 20 & \textbf{80} & 14       \\
        $\hyperref[fig:2_sync]{[3 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/3_sync.png}  & 10 & 30 & \textbf{80} & 24  \\
        $\hyperref[fig:3_sync]{[4 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/4_sync.png}  & 0 & 10 & \textbf{40} & 10 \\
        $\hyperref[fig:4_sync]{[5 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/5_sync.png}  & 0 & 0 & \textbf{60} & 15 \\
        $\hyperref[fig:5_sync]{[6 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/6_sync.png}  & 10 & \textbf{20} & \textbf{20} & 23 \\
        $\hyperref[fig:6_sync]{[7 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/7_sync.png}  & 0 & 0 & \textbf{50} & 36 \\
        $\hyperref[fig:7_sync]{[8 ]}$ \includegraphics[width=1cm]{assets/task_specific_assets/8_sync.png}  & 0 & 10 & \textbf{30} & 44 \\
        $\hyperref[fig:8_sync]{[9 ]}$ \includegraphics[width=1cm]{assets/task_specific_assets/9_sync.png}  & 0 & 10 & \textbf{20} & 63 \\
        $\hyperref[fig:9_sync]{[10]}$ \includegraphics[width=1cm]{assets/task_specific_assets/10_sync.png} & 0 & 0 & \textbf{20} & 57 \\
        \midrule
        \textbf{Total}   & 4 & 14 & \textbf{47} & \\
        \addlinespace[0.5em]
        \midrule
        \multicolumn{5}{c}{\textbf{Asynchronous}} \\
        \midrule
        $\hyperref[fig:0_async]{[1 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/1_async.png} & 10 & 0 & \textbf{20} & 21       \\
        $\hyperref[fig:1_async]{[2 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/2_async.png} & 0 & 0 & \textbf{30} & 27      \\
        $\hyperref[fig:2_async]{[3 ]}$ \includegraphics[width=0.5cm]{assets/task_specific_assets/3_async.png} & 0 & 0 & \textbf{40} & 37      \\
        $\hyperref[fig:3_async]{[4 ]}$ \includegraphics[width=1cm]{assets/task_specific_assets/4_async.png} & 0 & 0 & \textbf{10} & 42      \\
        $\hyperref[fig:4_async]{[5 ]}$ \includegraphics[width=1cm]{assets/task_specific_assets/5_async.png} & 0 & \textbf{10} & 0 & 46 \\
        $\hyperref[fig:5_async]{[6 ]}$ \includegraphics[width=1cm]{assets/task_specific_assets/6_async.png} & 0 & 0 & \textbf{10} & 19      \\
        $\hyperref[fig:6_async]{[7 ]}$ \includegraphics[width=2cm]{assets/task_specific_assets/7_async.png} & 0 & 0 & 0 & 42      \\
        $\hyperref[fig:7_async]{[8 ]}$ \includegraphics[width=1.5cm]{assets/task_specific_assets/8_async.png} & 0 & 0 & 0 & 46      \\
        $\hyperref[fig:8_async]{[9 ]}$ \includegraphics[width=2.5cm]{assets/task_specific_assets/9_async.png} & 0 & 0 & 0 & 68      \\
        $\hyperref[fig:9_async]{[10]}$ \includegraphics[width=2.5cm]{assets/task_specific_assets/10_async.png} & 0 & 0 & 0 & 82      \\
        \midrule
        \textbf{Total}   & 1 & 1 & \textbf{11} & \\
        \addlinespace[0.5em]
        \bottomrule
    \end{tabular}
    \caption{\gptfo{} performance on the synchronous and asynchronous datasets.}
    \label{tab:tasks-results}
\end{table}

==> prompts/io_example_async.tex <==
Interaction 1
---------------


Observation:
Station table1:
table1 is a table
table1 has bread1
table1 has bread1 directly on top of it
table1 has no players at it

Station board1:
board1 is a cutting board
board1 has lettuce1
board1 has lettuce1 directly on top of it
board1 has no players at it

Station sink1:
sink1 is a sink
sink1 has nothing on it
sink1 has no players at it

Station table2:
table2 is a table
table2 is occupied by robot1
table2 has chicken1
table2 has chicken1 directly on top of it

Station fryer1:
fryer1 is a fryer
fryer1 has nothing on it
fryer1 has no players at it

Station table3:
table3 is a table
table3 has nothing on it
table3 has no players at it

Station stove1:
stove1 is a stove
stove1 has nothing on it
stove1 has no players at it

Station sink2:
sink2 is a sink
sink2 has potato1
sink2 has potato1 directly on top of it
sink2 has no players at it

Station sink3:
sink3 is a sink
sink3 has onion1
sink3 has onion1 directly on top of it
sink3 has no players at it

Station fryer2:
fryer2 is a fryer
fryer2 has bread2
fryer2 has bread2 directly on top of it
fryer2 has no players at it

Station sink4:
sink4 is a sink
sink4 has onion2
sink4 has onion2 directly on top of it
sink4 has no players at it

Station board2:
board2 is a cutting board
board2 has nothing on it
board2 has no players at it

Item bread1:
bread1 is a bread slice
bread1 is at table1
bread1 is directly on top of table1
bread1 has nothing above it

Item lettuce1:
lettuce1 is a head of lettuce
lettuce1 can be cut on a cutting board
lettuce1 is at board1
lettuce1 is directly on top of board1
lettuce1 has nothing above it

Item chicken1:
chicken1 is a chicken breast
chicken1 can be cooked on a stove
chicken1 is at table2
chicken1 is directly on top of table2
chicken1 has nothing above it

Item potato1:
potato1 is a potato
potato1 is at sink2
potato1 is directly on top of sink2
potato1 has nothing above it

Item onion1:
onion1 is an onion
onion1 can be cut on a cutting board
onion1 is at sink3
onion1 is directly on top of sink3
onion1 has nothing above it

Item bread2:
bread2 is a bread slice
bread2 is at fryer2
bread2 is directly on top of fryer2
bread2 has nothing above it

Item onion2:
onion2 is an onion
onion2 can be cut on a cutting board
onion2 is at sink4
onion2 is directly on top of sink4
onion2 has nothing above it

Player robot1:
robot1 is a robot
robot1 is at table2
robot1 is holding nothing

Valid Actions:
Move robot1 from table2 to table1
Move robot1 from table2 to board1
Move robot1 from table2 to sink1
Move robot1 from table2 to fryer1
Move robot1 from table2 to table3
Move robot1 from table2 to stove1
Move robot1 from table2 to sink2
Move robot1 from table2 to sink3
Move robot1 from table2 to fryer2
Move robot1 from table2 to sink4
Move robot1 from table2 to board2
Pick up chicken1 from table2 using robot1
Do nothing

Goal: Prepare an onion chicken sandwich on a table


Plan:
Pick up chicken1 from table2 using robot1
Move robot1 from table2 to stove1
Place chicken1 on stove1 using robot1
Cook chicken1 on stove1 using robot1
Move robot1 from stove1 to sink4
Pick up onion2 from sink4 using robot1
Move robot1 from sink4 to board2
Place onion2 on board2 using robot1
Cut onion2 on board2 using robot1
Cut onion2 on board2 using robot1
Cut onion2 on board2 using robot1
Pick up onion2 from board2 using robot1
Move robot1 from board2 to table1
Stack onion2 on top of bread1 using robot1
Move robot1 from table1 to stove1
Pick up chicken1 from stove1 using robot1
Move robot1 from stove1 to table1
Stack chicken1 on top of onion2 using robot1
Move robot1 from table1 to fryer2
Pick up bread2 from fryer2 using robot1
Move robot1 from fryer2 to table1
Stack bread2 on top of chicken1 using robot1

==> prompts/io_example_sync.tex <==
Interaction 1
---------------


Observation:
Station table1:
table1 is a table
table1 has bread1
table1 has bread1 directly on top of it
table1 has no players at it

Station board1:
board1 is a cutting board
board1 has lettuce1
board1 has lettuce1 directly on top of it
board1 has no players at it

Station sink1:
sink1 is a sink
sink1 has nothing on it
sink1 has no players at it

Station stove1:
stove1 is a stove
stove1 is occupied by robot1
stove1 has bread2
stove1 has bread2 directly on top of it

Station fryer1:
fryer1 is a fryer
fryer1 has onion1
fryer1 has onion1 directly on top of it
fryer1 has no players at it

Station table2:
table2 is a table
table2 has nothing on it
table2 has no players at it

Station board2:
board2 is a cutting board
board2 has bottombun1
board2 has bottombun1 directly on top of it
board2 has no players at it

Station table3:
table3 is a table
table3 has nothing on it
table3 has no players at it

Station sink2:
sink2 is a sink
sink2 has potato1
sink2 has potato1 directly on top of it
sink2 has no players at it

Station sink3:
sink3 is a sink
sink3 has cheese1
sink3 has cheese1 directly on top of it
sink3 has no players at it

Station sink4:
sink4 is a sink
sink4 has onion2
sink4 has onion2 directly on top of it
sink4 has no players at it

Station fryer2:
fryer2 is a fryer
fryer2 has nothing on it
fryer2 has no players at it

Item bread1:
bread1 is a bread slice
bread1 is at table1
bread1 is directly on top of table1
bread1 has nothing above it

Item lettuce1:
lettuce1 is a head of lettuce
lettuce1 can be cut on a cutting board
lettuce1 is at board1
lettuce1 is directly on top of board1
lettuce1 has nothing above it

Item bread2:
bread2 is a bread slice
bread2 is at stove1
bread2 is directly on top of stove1
bread2 has nothing above it

Item onion1:
onion1 is an onion
onion1 can be cut on a cutting board
onion1 is at fryer1
onion1 is directly on top of fryer1
onion1 has nothing above it

Item bottombun1:
bottombun1 is a bottom bun
bottombun1 is at board2
bottombun1 is directly on top of board2
bottombun1 has nothing above it

Item potato1:
potato1 is a potato
potato1 is at sink2
potato1 is directly on top of sink2
potato1 has nothing above it

Item cheese1:
cheese1 is a cheese slice
cheese1 is at sink3
cheese1 is directly on top of sink3
cheese1 has nothing above it

Item onion2:
onion2 is an onion
onion2 can be cut on a cutting board
onion2 is at sink4
onion2 is directly on top of sink4
onion2 has nothing above it

Player robot1:
robot1 is a robot
robot1 is at stove1
robot1 is holding nothing

Valid Actions:
Move robot1 from stove1 to table1
Move robot1 from stove1 to board1
Move robot1 from stove1 to sink1
Move robot1 from stove1 to fryer1
Move robot1 from stove1 to table2
Move robot1 from stove1 to board2
Move robot1 from stove1 to table3
Move robot1 from stove1 to sink2
Move robot1 from stove1 to sink3
Move robot1 from stove1 to sink4
Move robot1 from stove1 to fryer2
Pick up bread2 from stove1 using robot1
Do nothing

Goal: Prepare a onion cheese sandwich on a table


Plan:
Move robot1 from stove1 to board1
Pick up lettuce1 from board1 using robot1
Move robot1 from board1 to table3
Place lettuce1 on table3 using robot1
Move robot1 from table3 to fryer1
Pick up onion1 from fryer1 using robot1
Move robot1 from fryer1 to board1
Place onion1 on board1 using robot1
Cut onion1 on board1 using robot1
Cut onion1 on board1 using robot1
Cut onion1 on board1 using robot1
Pick up onion1 from board1 using robot1
Move robot1 from board1 to table1
Stack onion1 on top of bread1 using robot1
Move robot1 from table1 to sink3
Pick up cheese1 from sink3 using robot1
Move robot1 from sink3 to table1
Stack cheese1 on top of onion1 using robot1
Move robot1 from table1 to stove1
Pick up bread2 from stove1 using robot1
Move robot1 from stove1 to table1
Stack bread2 on top of cheese1 using robot1

==> prompts/io_prompt.tex <==
You must propose a plan given an observation and valid actions.

You will receive the initial state and the goal as follows:
    Optional[Error Feedback: ...]
    Observation: ...
    Valid Actions: ...

where
    - 'Observation' contains state information about objects in the environment and the goal
    - 'Valid Actions' is the list of actions you can take in the current state
    - 'Error Feedback' includes feedback about an invalid action taken in the previous interaction

Always format your response as follows:
Plan: ...

where:
    - 'Plan' is the sequence of actions you propose to take in the environment to reach the goal
    - The actions should be formatted exactly as they are in the environment description
    - Do not include any numbering or bullet points for the actions

Below is a description of the environment:
You are a robot in a kitchen environment. The objects in the kitchen and your goal are described in the Observation. The various types of objects in the kitchen include
    - Station: A location in the kitchen where you can perform special actions, e.g. cooking or cutting
    - Item: An object that can be picked up and potentially used in a Station
    - Player: Robots, including you, that are present in the kitchen
    - Container: An object that can hold other objects, e.g. a pot or a pan
    - Meal: A mixture of ingredients contained within a Container

The rules of the environment are as follows:
    - A Player can only hold a single Item at a time
    - An Item must be placed on a Station to perform an action on it
    - A Station must contain a single Item to perform an action on it
    - Items can only be stacked on top of one another
    - A Container can hold multiple Items
    - A Meal can be transferred between Containers

The goal of this environment is to satisfy a human's request, such as 'make me a hamburger'. These goals are intentionally underspecified so common sense reasoning is required to complete them. Specifically, it is important to consider
    - the minimal ingredients required to satisfy the request
    - any preparation steps for the ingredients like cooking, cutting, etc.

When the goal is achieved or a time limit is reached, the environment will end.

Follow this recipe guide to learn how to make food in Robotouille:
    Sandwich - A slice of bread, stacked on prepared ingredients, stacked on another slice of bread.
    Hamburger - A bottom bun, stacked on prepared ingredients, stacked on a top bun.
    Soup - A pot of boiling water containing prepared ingredients served in a bowl.

The actions you can take in the environment are as follows:
    - Move {p1} from {s1} to {s2} | Moves Player {p1} from Station {s1} to Station {s2}
    - Pick up {i1/c1} from {s1} using {p1} | Picks up Item {i1} or Container {c1} from Station {s1} using Player {p1}
    - Place {i1/c1} on {s1} using {p1} | Places Item {i1} or Container {c1} on Station {s1} using Player {p1}
    - Stack {i1} on top of {i2} using {p1} | Stacks Item {i1} on top of Item {i2} using Player {p1}
    - Unstack {i1} from {i2} using {p1} | Unstacks Item {i1} from Item {i2} using Player {p1}
    - Cook {i1} on {s1} using {p1} | Cooks Item {i1} on Station {s1} using Player {p1} (fully cooks over 3 timesteps, not immediate)
    - Cut {i1} on {s1} using {p1} | Cuts Item {i1} on Station {s1} using Player {p1} (must cut 3 times in succession, not immediate)
    - Fry {i1} on {s1} using {p1} | Fries Item {i1} on Station {s1} using Player {p1} (fully fries over 3 timesteps, not immediate)
    - Fill {c1} with water from {s1} using {p1} | Fills Container {c1} with water from Station {s1} using Player {p1}
    - Boil {c1}'s contents on {s1} using {p1} | Boils the contents of Container {c1} on Station {s1} using Player {p1} (fully boils over 3 timesteps, not immediate)
    - Add {i1} into {c1} using {p1} | Adds Item {i1} into Container {c1} using Player {p1}
    - Fill {c1} with {c2}'s contents using {p1} | Fills Container {c1} with the contents of Container {c2} using Player {p1}
    - Do nothing | Takes no action, consumes 1 timestep

==> prompts/iocot_example_async.tex <==
Interaction 1
---------------


Observation:
Station table1:
table1 is a table
table1 has bread1
table1 has bread1 directly on top of it
table1 has no players at it

Station board1:
board1 is a cutting board
board1 has lettuce1
board1 has lettuce1 directly on top of it
board1 has no players at it

Station sink1:
sink1 is a sink
sink1 has nothing on it
sink1 has no players at it

Station table2:
table2 is a table
table2 is occupied by robot1
table2 has chicken1
table2 has chicken1 directly on top of it

Station fryer1:
fryer1 is a fryer
fryer1 has nothing on it
fryer1 has no players at it

Station table3:
table3 is a table
table3 has nothing on it
table3 has no players at it

Station stove1:
stove1 is a stove
stove1 has nothing on it
stove1 has no players at it

Station sink2:
sink2 is a sink
sink2 has potato1
sink2 has potato1 directly on top of it
sink2 has no players at it

Station sink3:
sink3 is a sink
sink3 has onion1
sink3 has onion1 directly on top of it
sink3 has no players at it

Station fryer2:
fryer2 is a fryer
fryer2 has bread2
fryer2 has bread2 directly on top of it
fryer2 has no players at it

Station sink4:
sink4 is a sink
sink4 has onion2
sink4 has onion2 directly on top of it
sink4 has no players at it

Station board2:
board2 is a cutting board
board2 has nothing on it
board2 has no players at it

Item bread1:
bread1 is a bread slice
bread1 is at table1
bread1 is directly on top of table1
bread1 has nothing above it

Item lettuce1:
lettuce1 is a head of lettuce
lettuce1 can be cut on a cutting board
lettuce1 is at board1
lettuce1 is directly on top of board1
lettuce1 has nothing above it

Item chicken1:
chicken1 is a chicken breast
chicken1 can be cooked on a stove
chicken1 is at table2
chicken1 is directly on top of table2
chicken1 has nothing above it

Item potato1:
potato1 is a potato
potato1 is at sink2
potato1 is directly on top of sink2
potato1 has nothing above it

Item onion1:
onion1 is an onion
onion1 can be cut on a cutting board
onion1 is at sink3
onion1 is directly on top of sink3
onion1 has nothing above it

Item bread2:
bread2 is a bread slice
bread2 is at fryer2
bread2 is directly on top of fryer2
bread2 has nothing above it

Item onion2:
onion2 is an onion
onion2 can be cut on a cutting board
onion2 is at sink4
onion2 is directly on top of sink4
onion2 has nothing above it

Player robot1:
robot1 is a robot
robot1 is at table2
robot1 is holding nothing

Valid Actions:
Move robot1 from table2 to table1
Move robot1 from table2 to board1
Move robot1 from table2 to sink1
Move robot1 from table2 to fryer1
Move robot1 from table2 to table3
Move robot1 from table2 to stove1
Move robot1 from table2 to sink2
Move robot1 from table2 to sink3
Move robot1 from table2 to fryer2
Move robot1 from table2 to sink4
Move robot1 from table2 to board2
Pick up chicken1 from table2 using robot1
Do nothing

Goal: Prepare an onion chicken sandwich on a table


Action: Pick up chicken1 from table2 using robot1
Next State Change: chicken1 is held by robot1, chicken1 is not at table2
Action: Move robot1 from table2 to stove1
Next State Change: robot1 is at stove1, robot1 is not at table2
Action: Place chicken1 on stove1 using robot1
Next State Change: chicken1 is at stove1, chicken1 is not held by robot1
Action: Cook chicken1 on stove1 using robot1
Next State Change: chicken1 has started to cook
Action: Move robot1 from stove1 to sink4
Next State Change: chicken1 is cooking (3), robot1 is at sink4, robot1 is not at stove1
Action: Pick up onion2 from sink4 using robot1
Next State Change: chicken1 is cooking (2), onion2 is held by robot1, onion2 is not at sink4
Action: Move robot1 from sink4 to board2
Next State Change: chicken1 is cooking (1), robot1 is at board2, robot1 is not at sink4
Action: Place onion2 on board2 using robot1
Next State Change: chicken1 is cooked, onion2 is on board2, onion2 is not held by robot1
Action: Cut onion2 on board2 using robot1
Next State Change: onion2 is being cut (2)
Action: Cut onion2 on board2 using robot1
Next State Change: onion2 is being cut (1)
Action: Cut onion2 on board2 using robot1
Next State Change: onion2 is cut
Action: Pick up onion2 from board2 using robot1
Next State Change: onion2 is held by robot1, onion2 is not on board2
Action: Move robot1 from board2 to table1
Next State Change: robot1 is at table1, robot1 is not at board2
Action: Stack onion2 on top of bread1 using robot1
Next State Change: onion2 is atop bread1, onion2 is not held by robot1
Action: Move robot1 from table1 to stove1
Next State Change: robot1 is at stove1, robot1 is not at table1
Action: Pick up chicken1 from stove1 using robot1
Next State Change: chicken1 is held by robot1, chicken1 is not at stove1
Action: Move robot1 from stove1 to table1
Next State Change: robot1 is at table1, robot1 is not at stove1
Action: Stack chicken1 on top of onion2 using robot1
Next State Change: chicken1 is atop onion2, chicken1 is not held by robot1
Action: Move robot1 from table1 to fryer2
Next State Change: robot1 is at fryer2, robot1 is not at table1
Action: Pick up bread2 from fryer2 using robot1
Next State Change: bread2 is held by robot1, bread2 is not at fryer2
Action: Move robot1 from fryer2 to table1
Next State Change: robot1 is at table1, robot1 is not at fryer2
Action: Stack bread2 on top of chicken1 using robot1
Next State Change: bread2 is atop chicken1, bread2 is not held by robot1. Goal achieved!

==> prompts/iocot_example_sync.tex <==
Interaction 1
---------------


Observation:
Station table1:
table1 is a table
table1 has bread1
table1 has bread1 directly on top of it
table1 has no players at it

Station board1:
board1 is a cutting board
board1 has lettuce1
board1 has lettuce1 directly on top of it
board1 has no players at it

Station sink1:
sink1 is a sink
sink1 has nothing on it
sink1 has no players at it

Station stove1:
stove1 is a stove
stove1 is occupied by robot1
stove1 has bread2
stove1 has bread2 directly on top of it

Station fryer1:
fryer1 is a fryer
fryer1 has onion1
fryer1 has onion1 directly on top of it
fryer1 has no players at it

Station table2:
table2 is a table
table2 has nothing on it
table2 has no players at it

Station board2:
board2 is a cutting board
board2 has bottombun1
board2 has bottombun1 directly on top of it
board2 has no players at it

Station table3:
table3 is a table
table3 has nothing on it
table3 has no players at it

Station sink2:
sink2 is a sink
sink2 has potato1
sink2 has potato1 directly on top of it
sink2 has no players at it

Station sink3:
sink3 is a sink
sink3 has cheese1
sink3 has cheese1 directly on top of it
sink3 has no players at it

Station sink4:
sink4 is a sink
sink4 has onion2
sink4 has onion2 directly on top of it
sink4 has no players at it

Station fryer2:
fryer2 is a fryer
fryer2 has nothing on it
fryer2 has no players at it

Item bread1:
bread1 is a bread slice
bread1 is at table1
bread1 is directly on top of table1
bread1 has nothing above it

Item lettuce1:
lettuce1 is a head of lettuce
lettuce1 can be cut on a cutting board
lettuce1 is at board1
lettuce1 is directly on top of board1
lettuce1 has nothing above it

Item bread2:
bread2 is a bread slice
bread2 is at stove1
bread2 is directly on top of stove1
bread2 has nothing above it

Item onion1:
onion1 is an onion
onion1 can be cut on a cutting board
onion1 is at fryer1
onion1 is directly on top of fryer1
onion1 has nothing above it

Item bottombun1:
bottombun1 is a bottom bun
bottombun1 is at board2
bottombun1 is directly on top of board2
bottombun1 has nothing above it

Item potato1:
potato1 is a potato
potato1 is at sink2
potato1 is directly on top of sink2
potato1 has nothing above it

Item cheese1:
cheese1 is a cheese slice
cheese1 is at sink3
cheese1 is directly on top of sink3
cheese1 has nothing above it

Item onion2:
onion2 is an onion
onion2 can be cut on a cutting board
onion2 is at sink4
onion2 is directly on top of sink4
onion2 has nothing above it

Player robot1:
robot1 is a robot
robot1 is at stove1
robot1 is holding nothing

Valid Actions:
Move robot1 from stove1 to table1
Move robot1 from stove1 to board1
Move robot1 from stove1 to sink1
Move robot1 from stove1 to fryer1
Move robot1 from stove1 to table2
Move robot1 from stove1 to board2
Move robot1 from stove1 to table3
Move robot1 from stove1 to sink2
Move robot1 from stove1 to sink3
Move robot1 from stove1 to sink4
Move robot1 from stove1 to fryer2
Pick up bread2 from stove1 using robot1
Do nothing

Goal: Prepare a onion cheese sandwich on a table


Action: Move robot1 from stove1 to board1
Next State Change: robot1 is at board1, robot1 is not at stove1
Action: Pick up lettuce1 from board1 using robot1
Next State Change: lettuce1 is held by robot1, lettuce1 is not at board1
Action: Move robot1 from board1 to table3
Next State Change: robot1 is at table3, robot1 is not at board1
Action: Place lettuce1 on table3 using robot1
Next State Change: lettuce1 is at table3, lettuce1 is not held by robot1
Action: Move robot1 from table3 to fryer1
Next State Change: robot1 is at fryer1, robot1 is not at table3
Action: Pick up onion1 from fryer1 using robot1
Next State Change: onion1 is held by robot1, onion1 is not at fryer1
Action: Move robot1 from fryer1 to board1
Next State Change: robot1 is at board1, robot1 is not at fryer1
Action: Place onion1 on board1 using robot1
Next State Change: onion1 is on board1, onion1 is not held by robot1
Action: Cut onion1 on board1 using robot1
Next State Change: onion1 is being cut (2)
Action: Cut onion1 on board1 using robot1
Next State Change: onion1 is being cut (1)
Action: Cut onion1 on board1 using robot1
Next State Change: onion1 has been cut
Action: Pick up onion1 from board1 using robot1
Next State Change: onion1 is held by robot1, onion1 is not at board1
Action: Move robot1 from board1 to table1
Next State Change: robot1 is at table1, robot1 is not at board1
Action: Stack onion1 on top of bread1 using robot1
Next State Change: onion1 is atop bread1, onion1 is not held by robot1
Action: Move robot1 from table1 to sink3
Next State Change: robot1 is at sink3, robot1 is not at table1
Action: Pick up cheese1 from sink3 using robot1
Next State Change: cheese1 is held by robot1, cheese1 is not at sink3
Action: Move robot1 from sink3 to table1
Next State Change: robot1 is at table1, robot1 is not at sink3
Action: Stack cheese1 on top of onion1 using robot1
Next State Change: cheese1 is atop onion1, cheese1 is not held by robot1
Action: Move robot1 from table1 to stove1
Next State Change: robot1 is at stove1, robot1 is not at table1
Action: Pick up bread2 from stove1 using robot1
Next State Change: bread2 is held by robot1, bread2 is not at stove1
Action: Move robot1 from stove1 to table1
Next State Change: robot1 is at table1, robot1 is not at stove1
Action: Stack bread2 on top of cheese1 using robot1
Next State Change: bread2 is atop cheese1, bread2 is not held by robot1. Goal achieved!

==> prompts/iocot_prompt.tex <==
You must propose a plan given an observation and valid actions.

You will receive the initial state and the goal as follows:
    Optional[Error Feedback: ...]
    Observation: ...
    Valid Actions: ...

where
    - 'Observation' contains state information about objects in the environment and the goal
    - 'Valid Actions' is the list of actions you can take in the current state
    - 'Error Feedback' includes feedback about an invalid action taken in the previous interaction

Always format your response as follows:
    Action: ...
    Next State Changes: ...
    Action: ...
    Next State Changes: ...
    ...

where:
    - 'Action' is the action you propose to take in the last state to reach the goal
    - The action should be formatted exactly as they are in the environment description
    - 'Next State' is the state after the action is taken
    - The state can be a summary of the changes in the environment after the action is taken 

Below is a description of the environment:
You are a robot in a kitchen environment. The objects in the kitchen and your goal are described in the Observation. The various types of objects in the kitchen include
    - Station: A location in the kitchen where you can perform special actions, e.g. cooking or cutting
    - Item: An object that can be picked up and potentially used in a Station
    - Player: Robots, including you, that are present in the kitchen
    - Container: An object that can hold other objects, e.g. a pot or a pan
    - Meal: A mixture of ingredients contained within a Container

The rules of the environment are as follows:
    - A Player can only hold a single Item at a time
    - An Item must be placed on a Station to perform an action on it
    - A Station must contain a single Item to perform an action on it
    - Items can only be stacked on top of one another
    - A Container can hold multiple Items
    - A Meal can be transferred between Containers

The goal of this environment is to satisfy a human's request, such as 'make me a hamburger'. These goals are intentionally underspecified so common sense reasoning is required to complete them. Specifically,
    it is important to consider
    - the minimal ingredients required to satisfy the request
    - any preparation steps for the ingredients like cooking, cutting, etc.

When the goal is achieved or a time limit is reached, the environment will end.

Follow this recipe guide to learn how to make food in Robotouille:
    Sandwich - A slice of bread, stacked on prepared ingredients, stacked on another slice of bread.
    Hamburger - A bottom bun, stacked on prepared ingredients, stacked on a top bun.
    Soup - A pot of boiling water containing prepared ingredients served in a bowl.

The actions you can take in the environment are as follows:
    - Move {p1} from {s1} to {s2} | Moves Player {p1} from Station {s1} to Station {s2}
    - Pick up {i1/c1} from {s1} using {p1} | Picks up Item {i1} or Container {c1} from Station {s1} using Player {p1}
    - Place {i1/c1} on {s1} using {p1} | Places Item {i1} or Container {c1} on Station {s1} using Player {p1}
    - Stack {i1} on top of {i2} using {p1} | Stacks Item {i1} on top of Item {i2} using Player {p1}
    - Unstack {i1} from {i2} using {p1} | Unstacks Item {i1} from Item {i2} using Player {p1}
    - Cook {i1} on {s1} using {p1} | Cooks Item {i1} on Station {s1} using Player {p1} (fully cooks over 3 timesteps, not immediate)
    - Cut {i1} on {s1} using {p1} | Cuts Item {i1} on Station {s1} using Player {p1} (must cut 3 times in succession, not immediate)
    - Fry {i1} on {s1} using {p1} | Fries Item {i1} on Station {s1} using Player {p1} (fully fries over 3 timesteps, not immediate)
    - Fill {c1} with water from {s1} using {p1} | Fills Container {c1} with water from Station {s1} using Player {p1}
    - Boil {c1}'s contents on {s1} using {p1} | Boils the contents of Container {c1} on Station {s1} using Player {p1} (fully boils over 3 timesteps, not immediate)
    - Add {i1} into {c1} using {p1} | Adds Item {i1} into Container {c1} using Player {p1}
    - Fill {c1} with {c2}'s contents using {p1} | Fills Container {c1} with the contents of Container {c2} using Player {p1}
    - Do nothing | Takes no action, consumes 1 timestep

==> prompts/react_example_async.tex <==
Interaction 1
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. I see chicken1 on table2. I must pick it up and place it on a stove to cook it.

Action: Pick up chicken1 from table2 using robot1


Interaction 2
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. I am holding chicken1. I must place it on a stove to cook it. I see stove1 is empty. Thus, I will move to stove1.

Action: Move robot1 from table2 to stove1


Interaction 3
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. I am holding chicken1. I must place it on a stove to cook it. I am at stove1 which is empty. I will place chicken1 on stove1.

Action: Place chicken1 on stove1 using robot1


Interaction 4
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is on stove1. I must cook it before I can stack it on the sandwich.

Action: Cook chicken1 on stove1 using robot1


Interaction 5
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooking on stove1. Thus, I will leave it in place.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I will move to sink4 to pick up onion2.

Action: Move robot1 from stove1 to sink4


Interaction 6
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooking on stove1. Thus, I will leave it in place.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I will pickup onion2 from sink4 to cut it.

Action: Pick up onion2 from sink4 using robot1


Interaction 7
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooking on stove1. Thus, I will leave it in place.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and am holding onion2. I must cut an onion fully before I can stack it on top of bread1. onion2 can be cut on a cutting board. I see board1 has lettuce1 on it and board2 has nothing on it. I will move to board2 to cut onion2.

Action: Move robot1 from sink4 to board2


Interaction 8
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and am holding onion2. I must cut an onion fully before I can stack it on top of bread1. onion2 can be cut on a cutting board. I see board1 has lettuce1 on it and board2 has nothing on it. Since I am at board2, I will place onion2 on it to cut it.

Action: Place onion2 on board2 using robot1


Interaction 9
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and onion2 on board2. I must cut an onion fully before I can stack it on top of bread1. onion2 can be cut on a cutting board. I see board1 has lettuce1 on it and board2 has onion2 on it. Since I am at board2, I will cut onion2.

Action: Cut onion2 on board2 using robot1


Interaction 10
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and onion2 on board2. I must cut an onion fully before I can stack it on top of bread1. onion2 can be cut on a cutting board. I see board1 has lettuce1 on it and board2 has onion2 on it. Since I am at board2, I will continue to cut onion2.

Action: Cut onion2 on board2 using robot1


Interaction 11
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and onion2 on board2. I must cut an onion fully before I can stack it on top of bread1. onion2 can be cut on a cutting board. I see board1 has lettuce1 on it and board2 has onion2 on it. Since I am at board2, I will continue to cut onion2.

Action: Cut onion2 on board2 using robot1


Interaction 12
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and onion2 on board2. onion2 has already been cut and is on board2. I will pick up onion2 from board2 to stack it on top of bread1.

Action: Pick up onion2 from board2 using robot1


Interaction 13
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and am holding onion2. Since onion2 has already been cut, I will stack it on bread1 to build the sandwich. Since bread1 is on table1, I will move from board2 to table1 to stack onion2 on top of bread1.

Action: Move robot1 from board2 to table1


Interaction 14
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion1 on sink3 and am holding onion2. Since onion2 has already been cut and I am at table1 where bread1 currently is, I will stack onion2 on bread1 to build the sandwich.

Action: Stack onion2 on top of bread1 using robot1


Interaction 15
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I see chicken1 cooked and at stove1. I will move to stove1 to pick up chicken1 and then stack it on top of onion2.

Action: Move robot1 from table1 to stove1


Interaction 16
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 has already been cooked and is at stove1. Thus, I will leave it in place until I am ready to stack it on the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I am at stove1 where chicken1 has been cooked. I will pick up chicken1 and then stack it on top of onion2.

Action: Pick up chicken1 from stove1 using robot1


Interaction 17
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooked and is held by robot1.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I am holding chicken1 and must stack it on onion2. onion2 is at table1 so I will move from stove1 to table1 to stack chicken1 on top of onion2.

Action: Move robot1 from stove1 to table1


Interaction 18
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooked and is held by robot1.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I am holding chicken1 and am at table1 where onion2 is. I will stack chicken1 on top of onion2 to continue building the sandwich.

Action: Stack chicken1 on top of onion2 using robot1


Interaction 19
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooked and in the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I see chicken1 stacked on onion2. Since chicken1 is already stacked on onion2, I will leave it in place and move to the next step.

5. The fourth ingredient is bread. I see bread2 on fryer2. I will move from table1 to fryer2 to pick up bread2 and stack it on top of chicken1 to complete the sandwich.

Action: Move robot1 from table1 to fryer2


Interaction 20
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooked and in the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I see chicken1 stacked on onion2. Since chicken1 is already stacked on onion2, I will leave it in place and move to the next step.

5. The fourth ingredient is bread. I see bread2 on fryer2. Since I am at fryer2, I will pick up bread2 and stack it on top of chicken1 to complete the sandwich.

Action: Pick up bread2 from fryer2 using robot1


Interaction 21
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooked and in the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I see chicken1 stacked on onion2. Since chicken1 is already stacked on onion2, I will leave it in place and move to the next step.

5. The fourth ingredient is bread. I am holding bread2 and must stack bread2 on chicken1. Since I am at fryer2, I will move from fryer2 to table1 to stack bread2 on top of chicken1 to complete the sandwich.

Action: Move robot1 from fryer2 to table1


Interaction 22
---------------


Observation: ...

Valid Actions: ...

Goal: Prepare an onion chicken sandwich on a table


Reasoning: The goal is to make an onion chicken sandwich on a table. I can cook chicken while doing other tasks. Thus, I
will stack the ingredients from bottom to top as follows: table -> bread -> onion -> chicken -> bread.

1. First I will leave the chicken cooking. chicken1 is already cooked and in the sandwich.

2. The first ingredient is bread. I see bread1 on table1 and bread2 on fryer2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

3. The second ingredient is onion. I see onion2 stacked on bread1. Since onion2 is already stacked on bread1, I will leave it in place and move to the next step.

4. The third ingredient is chicken. I see chicken1 stacked on onion2. Since chicken1 is already stacked on onion2, I will leave it in place and move to the next step.

5. The fourth ingredient is bread. I am holding bread2 and must stack bread2 on chicken1. Since I am at table1, I will stack bread2 on top of chicken1 to complete the sandwich.

Action: Stack bread2 on top of chicken1 using robot1

==> prompts/react_example_sync.tex <==
Interaction 1
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on fryer1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 has lettuce1 on it and board2 has bottombun1 on it. The board must be empty before I can cut onion1 on it. I will move robot1 from stove1 to board1.

Action: Move robot1 from stove1 to board1


Interaction 2
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on fryer1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 has lettuce1 on it and board2 has bottombun1 on it. The board must be empty before I can cut onion1 on it. Since robot1 is at board1, I will pick up lettuce1 from board1 using robot1 and move it elsewhere.

Action: Pick up lettuce1 from board1 using robot1


Interaction 3
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on fryer1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 is empty and board2 has bottombun1 on it. Since board1 is empty, I will use it to cut onion1. Since robot1 is holding lettuce1 after clearing board1, I must move the lettuce to another location. table3 is empty, so I will move robot1 from board1 to table3 to place lettuce1 on it.

Action: Move robot1 from board1 to table3


Interaction 4
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on fryer1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 is empty and board2 has bottombun1 on it. Since board1 is empty, I will use it to cut onion1. Since robot1 is holding lettuce1 and can only hold one item at a time, I will place lettuce1 on table3 because it is empty and we are using neither table3 nor lettuce1 for the sandwich.

Action: Place lettuce1 on table3 using robot1


Interaction 5
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on fryer1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 is empty and board2 has bottombun1 on it. Since board1 is empty, I will use it to cut onion1. I will move robot1 from table3 to fryer1 to pick up onion1.

Action: Move robot1 from table3 to fryer1


Interaction 6
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on fryer1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 is empty and board2 has bottombun1 on it. Since robot1 is at fryer1, I will use it to pick up onion1 to cut at board1.

Action: Pick up onion1 from fryer1 using robot1


Interaction 7
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 held by robot1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 is empty and board2 has bottombun1 on it. Since robot1 is at fryer1 and holding onion1, I will move it to board1 to place and begin cutting the onion.

Action: Move robot1 from fryer1 to board1


Interaction 8
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 held by robot1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 and onion2 can be cut on a cutting board. I see board1 is empty and board2 has bottombun1 on it. Since robot1 is at board1 and holding onion1, I will place onion1 on board1 to begin cutting it.

Action: Place onion1 on board1 using robot1


Interaction 9
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on board1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. Since robot1 is at board1 and onion1 is on board1, I will use robot1 to cut onion1.

Action: Cut onion1 on board1 using robot1


Interaction 10
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on board1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. Since robot1 is at board1 and onion1 is on board1, I will use robot1 to cut onion1.

Action: Cut onion1 on board1 using robot1


Interaction 11
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on board1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. Since robot1 is at board1 and onion1 is on board1, I will use robot1 to cut onion1.

Action: Cut onion1 on board1 using robot1


Interaction 12
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 on board1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 is fully cut and ready to be stacked on top of bread1. Since robot1 is at board1 and onion1 is on board1, I will use robot1 to pick up onion1.

Action: Pick up onion1 from board1 using robot1


Interaction 13
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 held by robot1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 is fully cut and ready to be stacked on top of bread1. Since robot1 is holding onion1 and bread1 is on table1, I will move robot1 to table1 to stack onion1 on top of bread1.

Action: Move robot1 from board1 to table1


Interaction 14
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 held by robot1 and onion2 on sink4. I must cut an onion fully before I can stack it on top of bread1. onion1 is fully cut and ready to be stacked on top of bread1. Since robot1 is holding onion1 and at table1 and bread1 is on table1, I will use robot1 to to stack onion1 on top of bread1.

Action: Stack onion1 on top of bread1 using robot1


Interaction 15
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 on sink3. I must pick up cheese1 and stack it on top of onion1. Since robot1 is at table1 and cheese1 is on sink3, I will move robot1 to sink3 to pick up cheese1.

Action: Move robot1 from table1 to sink3


Interaction 16
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 on sink3. I must pick up cheese1 and stack it on top of onion1. Since robot1 is at sink3 and cheese1 is on sink3, I will use robot1 to pick up cheese1.

Action: Pick up cheese1 from sink3 using robot1


Interaction 17
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 held by robot1. I must stack cheese1 on top of onion1. Since robot1 is at sink3 and cheese1 is held by robot1, I will move robot1 to table1 to stack cheese1 on top of onion1.

Action: Move robot1 from sink3 to table1


Interaction 18
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 held by robot1. I must stack cheese1 on top of onion1. Since robot1 is at table1 and cheese1 is held by robot1, I will use robot1 to stack cheese1 on top of onion1.

Action: Stack cheese1 on top of onion1 using robot1


Interaction 19
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 stacked on onion1. I will leave it in place since it is already in the correct position.

4. The fourth ingredient is bread. I see bread2 on stove1. Since robot1 is at table1 and bread2 is on stove1, I will move robot1 to stove1 to pick up bread2.

Action: Move robot1 from table1 to stove1


Interaction 20
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 stacked on onion1. I will leave it in place since it is already in the correct position.

4. The fourth ingredient is bread. I see bread2 on stove1. Since robot1 is at table1 and bread2 is on stove1, I will move robot1 to stove1 to pick up bread2.

Action: Pick up bread2 from stove1 using robot1


Interaction 21
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 stacked on onion1. I will leave it in place since it is already in the correct position.

4. The fourth ingredient is bread. I see bread2 held by robot1. I must stack bread2 on top of cheese1. Since robot1 is holding bread2 and cheese1 is at table1, I will move robot1 to table1 to stack bread2 on top of cheese1.

Action: Move robot1 from stove1 to table1


Interaction 22
---------------


Observation:
...

Valid Actions:
...

Goal: Prepare a onion cheese sandwich on a table


Reasoning: The goal is to make an onion cheese sandwich on a table. I need ingredients stacked from bottom to top: table -> bread -> onion -> cheese -> bread

1. The first ingredient is bread. I see bread1 on table1 and bread2 on stove2. Since bread1 is on top of a table, it will serve as the base of the sandwich. I will leave it in place since it is already in the correct position.

2. The second ingredient is onion. I see onion1 stacked on bread1. onion1 is fully cut. I will leave it in place since it is already in the correct position.

3. The third ingredient is cheese. I see cheese1 stacked on onion1. I will leave it in place since it is already in the correct position.

4. The fourth ingredient is bread. I see bread2 held by robot1. I must stack bread2 on top of cheese1. Since robot1 is at table1 and bread2 is held by robot1, I will use robot1 to stack bread2 on top of cheese1.

Action: Stack bread2 on top of cheese1 using robot1

==> prompts/react_prior_prompt.tex <==
It is *important* to follow these rules before proposing an action:
    - A Player can pick up a single Item at a time
      - This means that you should not attempt to pick up an Item if you are already holding one
    - An Item must be placed on a Station to perform an action on it
      - This means that you cannot perform an action on an Item while holding it or if it is stacked on another Item at a Station
      - This also means that you must perform an action on an Item at a Station for state changes to occur (e.g. cooking)
    - A Station must contain a single Item to perform an action on it
      - This means that you can only bring an Item to a Station if it is already empty
    - Items can be stacked on top of one another
      - This means that Items are stacked on top of Items
    
    
    In addition, do not blindly follow these rules; think about how your actions will affect future actions since your plan may
    require you to break rules in the future to achieve the goal.

==> prompts/react_prompt.tex <==
You must propose an action given the current observation and valid actions and the last reasoning and action taken in the environment.

You will receive the initial state and the goal as follows:
    Optional[Error Feedback: ...]
    Observation: ...
    Valid Actions: ...

where
    - 'Observation' contains state information about objects in the environment and the goal
    - 'Valid Actions' is the list of actions you can take in the current state
    - 'Error Feedback' includes feedback about an invalid action taken in a previous interaction (not included in the history)
    - This feedback is automated and shows if the action is either syntactically incorrect or does not exist in the valid actions list
    - This feedback does not check for semantic correctness and should neither reinforce nor discourage the current strategy

Always format your response as follows:
    Reasoning: ...
    Action: ...

where:
    - 'Reasoning' includes reasoning about the action you will propose to take next
    - Incorporate the past reasoning and action into your current reasoning
    - Include a complete step by step action plan to the goal to justify the next action you'll propose to take 
    - 'Action' is the action you propose to take in the environment
    - This action should be formatted exactly as it is in the environment description
    - This should be the first action in the plan you created in the Reasoning section

Below is a description of the environment:
You are a robot in a kitchen environment. The objects in the kitchen and your goal are described in the Observation. The various types of objects in the kitchen include
    - Station: A location in the kitchen where you can perform special actions, e.g. cooking or cutting
    - Item: An object that can be picked up and potentially used in a Station
    - Player: Robots, including you, that are present in the kitchen
    - Container: An object that can hold meals, e.g. a pot or a pan
    - Meal: A mixture of ingredients contained within a Container

The rules of the environment are as follows:
    - A Player can only hold a single Item at a time
    - An Item must be placed on a Station to perform an action on it
    - A Station must contain a single Item to perform an action on it
    - Items can only be stacked on top of one another
    - A Container must contain a Meal to have items added to it
    - A Meal can be transferred between Containers

The goal of this environment is to satisfy a human's request, such as 'make me a hamburger'. These goals are intentionally underspecified so common sense reasoning is required to complete them. Specifically, it is important to consider
    - the minimal ingredients required to satisfy the request
    - any preparation steps for the ingredients like cooking, cutting, etc.

When the goal is achieved or a time limit is reached, the environment will end.

Follow this recipe guide to learn how to make food in Robotouille:
    Sandwich - A slice of bread, stacked on prepared ingredients, stacked on another slice of bread.
    Hamburger - A bottom bun, stacked on prepared ingredients, stacked on a top bun.
    Soup - A pot is first filled with water, then boiled while ingredients are added, then served in a bowl when ready.
